GPT-based Open-Ended Knowledge Tracing

In education applications, knowledge tracing refers to the problem of estimating students' time-varying concept/skill mastery level from their past responses to questions and predicting their future performance. One key limitation of most existing knowledge tracing methods is that they treat student responses to questions as binary-valued, i.e., whether they are correct or incorrect. Response correctness analysis/prediction ignores important information on student knowledge contained in the exact content of the responses, especially for open-ended questions. In this paper, we conduct the first exploration into open-ended knowledge tracing (OKT) by studying the new task of predicting students' exact open-ended responses to questions. Our work is grounded in the domain of computer science education with programming questions. We develop an initial solution to the OKT problem, a student knowledge-guided code generation approach, that combines program synthesis methods using language models with student knowledge tracing methods. We also conduct a series of quantitative and qualitative experiments on a real-world student code dataset to validate OKT and demonstrate its promise in educational applications.

==> recycle.tex <==
\section{The Open-Ended Knowledge Tracing Problem}

In this section, we introduce our novel open-ended knowledge tracing framework, henceforth referred to as OKT. We present various components in OKT, compare its problem setup with existing KT methods, and highlight the differences. 
%We then instantiate OKT for programming education which enables us to model students' code submissions in which answer correctness will no longer effectively suffice knowledge tracing. 
The OKT framework consists of three main components: 
\begin{enumerate}[a)]
\item \textbf{Knowledge representation}, which converts full question prompts/statements and open-ended student responses to continuous representations that are used as input to the knowledge update component. This component is different from most existing KT methods that only leverage question ID/response correctness-based representations except a few recent works: \citep{purdue,eernna} use word embeddings to represent question text while \citep{ncsupkt,pkt} use programming code embedding techniques to represent student code. 
\item \textbf{Knowledge update}, which updates the student's knowledge state after observing their response to a question. This component is the same as that for existing KT methods.
\item \textbf{Response generation}, which predicts the exact open-ended response of the student to an open-ended question using a domain-specific generative content model. The generation of (possibly long) open-ended response predictions makes OKT significantly different from existing KT methods whose response prediction components are simple binary classifiers. This component takes as input both the full question prompt and student knowledge states produced by the knowledge update component. 
%, in contrast to the generates the full based on a student's knowledge state and problem prompt using a generative model. 
\end{enumerate}

%The response generation component is where OKT significantly differs from the problem setting of existing KT methods. OKT predicts the exact (possibly long) response using generative models rather than only predicting a single binary-valued correctness label. Additionally, OKT uses the exact question content as input rather than learned question/concept embeddings mapped to . 
%There exist recently-developed KT methods that uses textual/code embedding techniques such as word2vec  and ASTNN/code2vec  to encode questions and/or student response, both for the knowledge representation component and as input to the response generation component, but none of these works use generative models to predict the exact student response. 

\sloppy
Figure~\ref{fig:okt} shows an illustration of the OKT framework. 
%By combining the three components, we formulate our problem setting as follows. 
Given a set of $N$ students, we denote each student's question-response record as $s^i = \{(p^i_1, x^i_1, y^i_1), \ldots, (p^i_{T_i}, x^i_{T_i}, y^i_{T_i})\}$, where the triple $(p^i_t, x^i_t, y^i_t)$ is student $i$'s response to a question at time step $t$ (a total of $T_i$ time steps). $p^i_t$ denotes the question prompt (often in the form of text but possibly contains other modalities such as mathematical/scientific symbols or code), $x^i_t$ is the student's open-ended response, and $y^i_t$ is its correctness (which we include for completeness of our problem formulation). 
% represents the total number of time steps, i.e., the number of attempts at questions, for student $i$. 
In what follows, for simplicity and clarity, we restrict our discussions to a single student and omit the student index $i$ unless necessary. Given a sequence of questions and responses from time step $1$ to time step $t-1$, $\{(p_1, x_1), \ldots, (p_{t-1}, x_{t-1})\}$, OKT aims to generate and predict open-ended student responses to future questions, starting with $x_t$ (rather than binary-valued response correctness $y_t$) at time step $t$. 
%Note that just like existing KT methods, we can also predict response correctness, $y_t$, but it is not required for OKT due to its open-ended nature. 
%; in some scenarios, one may also use $y_1, \ldots, y_{t-1}$ as input to the knowledge representation component, we discuss this scenario in Section~\ref{sec:kt}. 
%\nl{does this mean pre-trained LSTM? If so, it should be Section~\ref{sec:pre-train}} \ml{should be 3.2, but it's not really there either lol}



%For the sake of clarify, we will treat knowledge states as vectors here. Then with the above notations, we can describe our problem as follows: 
Formally, the OKT framework can be characterized as follows:

\begin{align}
    \begin{split}
    &\rvq_t = E_1(p_1, \ldots, p_t) \label{eq:1}\\
    &\rvc_t = E_2(x_1, \ldots, x_t)
    \end{split} \\
    &\rvh_t = \mathcal{KT} ((\rvq_1, \: \rvc_1, \: \rvh_1), \ldots, (\rvq_{t-1}, \: \rvc_{t-1}, \: \rvh_{t-1}), \rvq_t) \label{eq:2}\\
    &\hat{\rvx_t} = \mathcal{G} (\rvq_t, \rvh_t). \label{eq:3} 
\end{align} 
% \nl{there should be a time step mismatch for G?} \ml{good point - both are fine i think - depends on whether ht is the knowledge state before or after being updated by observing the code at time t. my notation is for before. some indices in the figure may need to change}
In Eq.~\ref{eq:1}, $\rvq$ and $\rvc$ denote the question and response representations, respectively, while $E_1$ and $E_2$ are their corresponding encoders in the knowledge representation component. In Eq.~\ref{eq:2}, $\mathcal{KT}$ is the knowledge update component and $\rvh_t$ represents the student's knowledge state at time step $t$, which is updated from previous questions, responses, and knowledge states using the current question representation. This formulation encompasses most existing KT methods: for latent variable-based BKT \citep{kt} and recurrent neural network-based DKT \citep{dkt}, $\rvq_t = E1(p_t), \rvc_t = E2(x_t), \rvh_t = \mathcal{KT} (\rvq_{t-1}, \rvc_{t-1}, \rvh_{t-1})$. For attention-based KT methods such as AKT \citep{akt}, the question/response representations are fully contextualized and the knowledge state is retrieved from these representations at all prior time steps. In Eq.~\ref{eq:3}, the response generation component $\mathcal{G}$ uses the student's current knowledge state $\rvh_{t}$ and question $\rvq_t$ to generate and predict the open-ended response $\hat{x_t}$. 
%\ml{i think here the following would further benefit this setup: first, i like the p and c formulation - it's more general and includes both the full attention and recurrent cases. for knowledge tracing, though, since traditional BKT techniques are recurrent, we may want to another equation here to highlight the recurrence aspect of things (as special cases to eqs 1 and 2 above). second, we should define what E, KT, and G are - i think giving them a name (encoder? knowledge tracer? generator?) would make it much more clear - even though we're describing a very generic framework here, we want to let the readers know how a typical BKT/DKT method fits into our framework.}
%
%The output of OKT, $\hat{x_t}$, is the predicted a student's open-ended response based on the already answered questions. This prediction allows us to directly compare the difference between generated answers and student answers, which gives us our loss function for a single student:
%We compare this predicted response against the student's actual open-ended response to arrive at our 

Most existing KT methods are optimized using the binary cross entropy loss due to the binary-valued prediction target ($y_t$). 
In contrast, in OKT, the components $E_1$, $E_2$, $\mathcal{KT}$, and $\mathcal{G}$ are jointly optimized through minimizing the OKT loss function
\begin{equation}
     Loss = \textstyle \sum_{i}\sum_{t} \ell (\rx_t, \: \hat{\rx_t})
\end{equation}
where $\ell$ is a domain-specific loss function comparing the predicted and actual student responses.

We emphasize that OKT is a general model that extends many existing KT methods to enable tracing and predictions of students' open-ended solutions. The choices of the three OKT components are highly flexible, enabling OKT to be applied to a wide range of real-world KT scenarios where open-ended solutions abound. In the remainder of this paper, we focus on a particular domain to demonstrate the utility of OKT but we emphasize that OKT applies broadly to many other domains. 
% \zw{added para; can del. if needed}
%suitable for the question's domain we detail a loss function for the domain of programming code in Section~\ref{sec:loss}. 
% Through minimizing the loss function, we can learn all (or some) parameters in all . 
%\nl{I think we don't update E1, E2 with this loss function?} \ml{in theory we can i think - say we fine-tune codebert as well during our training process. we're not doing it (let's mention this in the following section), but i think leaving the door open is better}
%In our setup, we use Cross-Entropy loss which calculates the negative log likelihood of the observed sequence of student responses under the model. 
%The model parameters are updated by optimizing knowledge tracing and answer generative model in Eq \ref{eq:2} and \ref{eq:3} simultaneously. We will lay out the details of the model architecture with an example of open-ended programming questions in the following section. 
%\nl{Loss function need advising!} \ml{i think it looks fine - it's generic and we can define what the loss is later. I'd say maybe remove the CE subscript from the equation? this way we can say you can put any loss function that is appropriate for the data format one wants to deal with. then we can say for almost every existing KT method, it's BCE because, well, you only predict binary-valued output}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/OKT-general.png}
    \caption{An illustration of the OKT framework.}
    \label{fig:okt}
    \vspace{-10pt}
\end{figure}
